QALM: Escaping Local Minima via Interleaved Exploration and Exploitation in Quantum Circuit Optimization

Quantum circuit optimizers face a fundamental limitation in how they tolerate temporary cost increases. At one extreme, greedy rule-based optimizers immediately apply any cost-reducing transformation, achieving high efficiency but quickly becoming trapped in local minima. At the other extreme, search-based optimizers accept cost-increasing moves to explore the circuit space and escape such minima. However, because search-based optimizers cannot determine within a reasonable time budget whether a given point is promising, that is, whether its neighborhood contains a deeper local minimum, they must blindly explore higher-cost regions. As a result, escaping the current basin to reach a promising point takes exponentially many steps. In this work, we show that this limitation can be overcome with a hybrid framework that interleaves the exhaustive exploration capabilities of search algorithms with the efficiency of rule-based optimization. We implement this framework as QALM, a novel optimizer designed to escape local minima without incurring the runtime penalties of pure search. Crucially, our results demonstrate that QALM does not merely strike a balance; it outperforms existing rule-based and search-based optimizers in circuit reduction rates while operating with the computational efficiency of rule-based systems. In a comprehensive evaluation across 248 circuits, QALM matches or exceeds the fidelity of the strongest baseline on 83.9% of these circuits, given the same time budget.

==> figtex/eval_2q.tex <==
\begin{table*}[ht]
\centering
\caption{Comparing \optName with existing optimizers on reducing $CX$ gate count for 10 minutes on the Nam gate set. ``PP'' denotes runs with \quartz's preprocessing pass. The best result for each circuit is in bold. \vspace{0.5em}}
\label{tab:eval_2q}
\begin{tabular}{l|rrrrrrr|r}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Circuit}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Orig.}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\voqc}}} & \multicolumn{1}{c}{\textbf{\voqc}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\queso}}} & \multicolumn{1}{c}{\textbf{\queso}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\guoq}}} & \multicolumn{1}{c|}{\textbf{\guoq}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\optName}}} \\
 &  &  & \multicolumn{1}{c}{\textbf{w/ PP}} &  & \multicolumn{1}{c}{\textbf{w/ PP}} &  & \multicolumn{1}{c|}{\textbf{w/ PP}} &  \\
\hline
\texttt{adder\_8} & 409 & 301 & 305 & 311 & 293 & 281 & 273 & \textbf{252} \\
\texttt{barenco\_tof\_3} & 24 & 18 & 18 & \textbf{16} & \textbf{16} & \textbf{16} & 18 & \textbf{16} \\
\texttt{barenco\_tof\_4} & 48 & 34 & 34 & 30 & 32 & 30 & 28 & \textbf{26} \\
\texttt{barenco\_tof\_5} & 72 & 50 & 50 & 44 & 48 & 44 & 47 & \textbf{38} \\
\texttt{barenco\_tof\_10} & 192 & 130 & 130 & \textbf{114} & 128 & 120 & \textbf{114} & 118 \\
\texttt{csla\_mux\_3} & 80 & 74 & 74 & 71 & 71 & 66 & 68 & \textbf{63} \\
\texttt{csum\_mux\_9} & 168 & 140 & 140 & 168 & \textbf{112} & 152 & 139 & 140 \\
\texttt{gf2\^{}4\_mult} & 99 & 99 & 99 & 99 & 97 & 89 & 90 & \textbf{84} \\
\texttt{gf2\^{}5\_mult} & 154 & 154 & 154 & 154 & 149 & 143 & 143 & \textbf{135} \\
\texttt{gf2\^{}6\_mult} & 221 & 221 & 221 & 221 & 214 & 217 & 200 & \textbf{190} \\
\texttt{gf2\^{}7\_mult} & 300 & 300 & 300 & 300 & 287 & 295 & 281 & \textbf{263} \\
\texttt{gf2\^{}8\_mult} & 405 & 405 & 405 & 405 & 405 & 399 & 379 & \textbf{361} \\
\texttt{gf2\^{}9\_mult} & 494 & 494 & 494 & 494 & 494 & 485 & 460 & \textbf{435} \\
\texttt{gf2\^{}10\_mult} & 609 & 609 & 609 & 609 & 609 & 602 & 580 & \textbf{536} \\
\texttt{mod5\_4} & 28 & 28 & 28 & 22 & 21 & \textbf{12} & 17 & 13 \\
\texttt{mod\_mult\_55} & 48 & 42 & 40 & 44 & 40 & \textbf{38} & 39 & \textbf{38} \\
\texttt{mod\_red\_21} & 105 & 81 & 79 & 79 & 81 & 78 & 82 & \textbf{74} \\
\texttt{qcla\_adder\_10} & 233 & 199 & 199 & 210 & 189 & 189 & 175 & \textbf{169} \\
\texttt{qcla\_com\_7} & 186 & 132 & 132 & 150 & 125 & 119 & 119 & \textbf{118} \\
\texttt{qcla\_mod\_7} & 382 & 328 & 314 & 356 & 308 & 317 & 294 & \textbf{283} \\
\texttt{rc\_adder\_6} & 93 & 71 & 71 & 81 & 71 & 72 & \textbf{69} & 71 \\
\texttt{tof\_3} & 18 & 14 & 14 & 14 & 14 & \textbf{12} & \textbf{12} & 14 \\
\texttt{tof\_4} & 30 & 22 & 22 & 22 & 22 & 22 & 22 & \textbf{18} \\
\texttt{tof\_5} & 42 & 30 & 30 & 30 & 30 & 30 & 28 & \textbf{24} \\
\texttt{tof\_10} & 102 & 70 & 70 & 70 & 70 & 66 & 71 & \textbf{56} \\
\texttt{vbe\_adder\_3} & 70 & 50 & 50 & 43 & 41 & 39 & 42 & \textbf{34} \\
\hline
\textbf{Geo. Mean Reduction} & -- & 17.1\% & 17.4\% & 18.1\% & 21.3\% & 24.5\% & 24.5\% & 30.2\% \\
\hline
\end{tabular}
\end{table*}

==> figtex/eval_quarl.tex <==
\begin{table}[t]
\centering
  \caption{Comparing \optName with \quarl with and without rotation merging on reducing gate count on the Nam gate set. We use \quarl's result numbers directly from their paper with a 6-hour time limit for each circuit. The best result for each circuit is in bold. \vspace{0.5em}}
  %\small
\begin{tabular}{l|rrr|r}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Circuit}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Orig.}}} & \multicolumn{1}{c}{\textbf{Quarl}} & \multicolumn{1}{c|}{\textbf{Quarl}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{QALM}}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{l}{\textbf{w/ PP}} & \multicolumn{1}{l|}{\textbf{w/o PP}} & \multicolumn{1}{c}{} \\ \hline
\texttt{tof\_3} & 45 & \textbf{33} & \textbf{33} & 35 \\
\texttt{barenco\_tof\_3} & 58 & \textbf{35} & 36 & 36 \\
\texttt{mod5\_4} & 63 & \textbf{24} & \textbf{24} & \textbf{24} \\
\texttt{tof\_4} & 75 & \textbf{51} & \textbf{51} & \textbf{51} \\
\texttt{barenco\_tof\_4} & 114 & \textbf{62} & \textbf{62} & \textbf{62} \\
\texttt{tof\_5} & 105 & \textbf{69} & \textbf{69} & \textbf{69} \\
\texttt{mod\_mult\_55} & 119 & \textbf{84} & \textbf{84} & 86 \\
\texttt{vbe\_adder\_3} & 150 & \textbf{71} & \textbf{71} & 73 \\
\texttt{barenco\_tof\_5} & 170 & \textbf{90} & 96 & 92 \\
\texttt{csla\_mux\_3} & 170 & 141 & 141 & \textbf{140} \\
\texttt{rc\_adder\_6} & 200 & \textbf{134} & 148 & 152 \\
\texttt{gf2\^{}4\_mult} & 225 & \textbf{160} & 163 & 165 \\
\texttt{tof\_10} & 255 & 169 & 169 & \textbf{159} \\
\texttt{mod\_red\_21} & 278 & 179 & \textbf{177} & \textbf{177} \\
\texttt{hwb6} & 259 & \textbf{193} & 196 & \textbf{193} \\
\texttt{gf2\^{}5\_mult} & 347 & \textbf{257} & 266 & 260 \\
\texttt{csum\_mux\_9} & 420 & \textbf{224} & 282 & 280 \\
\texttt{barenco\_tof\_10} & 450 & \textbf{236} & 274 & 244 \\
\texttt{qcla\_com\_7} & 443 & 258 & 277 & \textbf{252} \\
\texttt{ham15-low} & 443 & 323 & \textbf{322} & 325 \\
\texttt{gf2\^{}6\_mult} & 495 & \textbf{352} & 386 & 357 \\
\texttt{qcla\_adder\_10} & 521 & \textbf{380} & 391 & 383 \\
\texttt{gf2\^{}7\_mult} & 669 & \textbf{484} & 530 & 487 \\
\texttt{gf2\^{}8\_mult} & 883 & \textbf{648} & 755 & 641 \\
\texttt{qcla\_mod\_7} & 884 & 629 & 664 & \textbf{614} \\
\texttt{adder\_8} & 900 & 560 & 669 & \textbf{513} \\ \hline
\textbf{Geo. Mean (\%)} & -- & 35.8\% & 32.6\% & 34.9\% \\ \hline
\end{tabular}
  \label{tab:quarl}
\end{table}


==> figtex/eval_reduction_over_time.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figure/avg_reduction.pdf}
  \caption{Average gate count reduction over time. For \optName and \quartz, we save the gate count for each circuit after each iteration; for \queso and \guoq, we run them several times with different time limits to plot the lines.}
  \label{fig:reduction_over_time}
\end{figure}


